Spiking Cochlea with System-level Local Automatic Gain Control

Including local automatic gain control (AGC) circuitry into a silicon cochlea design has been challenging because of transistor mismatch and model complexity. To address this, we present an alternative system-level algorithm that implements channel-specific AGC in a silicon spiking cochlea by measuring the output spike activity of individual channels. The bandpass filter gain of a channel is adapted dynamically to the input amplitude so that the average output spike rate stays within a defined range. Because this AGC mechanism only needs counting and adding operations, it can be implemented at low hardware cost in a future design. We evaluate the impact of the local AGC algorithm on a classification task where the input signal varies over 32 dB input range. Two classifier types receiving cochlea spike features were tested on a speech versus noise classification task. The logistic regression classifier achieves an average of 6% improvement and 40.8% relative improvement in accuracy when the AGC is enabled. The deep neural network classifier shows a similar improvement for the AGC case and achieves a higher mean accuracy of 96% compared to the best accuracy of 91% from the logistic regression classifier.

==> tables/acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
\caption{Mean test accuracy of the LR and DNN classifiers on  all test amplitudes. Results are averaged over 6 runs.}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Training \\ Amplitude \big(mV$_{\textrm{RMS}}$\big)\end{tabular}}} & \multicolumn{4}{c|}{\textbf{Mean Test Accuracy (\%)}}                \\ \cline{2-5}  & \multicolumn{2}{c|}{\textbf{LR}} & \multicolumn{2}{c|}{\textbf{DNN}} \\ \cline{2-5} & \textbf{Non-AGC}  & \textbf{AGC} & \textbf{Non-AGC}  & \textbf{AGC}  \\ \hline
5   & 69.79 & 72.45  & 77.45  & 74.68         \\ \hline
10  & 77.98    & 82.38   & 84.16   & 84.88  \\ \hline
15  & 77.85   & 85.42   & 86.01  & 88.12  \\ \hline
50  & 71.77   & 84.64  & 85.39  & 91.31         \\ \hline
80  & 71.06 & 83.76   & 86.04   & 90.19    \\ \hline
all    & 85.25   & 91.28   & 94.73    & 96.07   \\ \hline
\end{tabular}
\label{tab:acc}
\end{table}

%5mV, 2.66%, 8.8% error impr, 0.03%, %10mV, 4.4%,20% error impr, 0.056%

%15mV, 7.57%, 34% rel impr
%50mV, 12.87%,45% relative im
%80mV, 12.7%, 43.9% improve
%all, 6.03%, 40.8% relative improvement 

%all, DNN,1.34% ,25.4 % relative improvement

==> tables/fpga_resource_utilization.tex <==
\begin{table}[!t]
\centering
\caption{Resource utilization of AGC control logic on FPGA LATTICE LFE$3$-$70$EA-$8$FN$484$C.}
\resizebox{0.5\textwidth}{!}{ % RESIZEBOX
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{}           & \textbf{LUT$4$} & \textbf{LUTRAM} & \textbf{FF} & \textbf{BRAM} ($18$Kb) & \textbf{DSP}   \\ \hline
\textbf{Available}  & $66528$         & $6804$            & $49896$       & $240$                  & $128$  \\ \hline
\textbf{Used}       & $5007$          & $48$              & $3217$        & $1$                    & $0$    \\ \hline
\textbf{Percentage} & $7.5$\%         & $0.7$\%           & $6.4$\%       & $0.4$\%                & $0$\%  \\ \hline
\end{tabular}
}
\label{tab:fpga_resource}
\end{table}



==> tables/freq_response.tex <==
% https://www.tablesgenerator.com
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[h]
\caption{Parameters of the channels used for frequency response measurement. $F_{ch}$ --- designed channel frequency, $F_m$ --- measured peak frequency, Freq sweep --- range of exponentially spaced frequencies used for frequency response measurements.}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Ch \#}  & \textbf{$\mathbf{F_{ch}}$, Hz} & \textbf{$\mathbf{F_m}$, Hz} & \textbf{Freq sweep, Hz} \\ \hline
$13$   & $3980$              & $4550$         & $400-8000$     \\ \hline
$23$   & $1150$              & $1500$         & $200-4000$     \\ \hline
$30$   & $482$               & $640$          & $100-2000$     \\ \hline
$36$   & $229$               & $290$          & $40-1000$      \\ \hline
$42$   & $109$               & $133$          & $40-1000$      \\ \hline
$48$   & $52$                & $58$           & $40-1000$      \\ \hline
\end{tabular}
\label{tab:freq_response}
\end{table}

==> tables/gain_settings.tex <==
% https://www.tablesgenerator.com
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Gain index\\ ($4$ bit)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Total Gain,\\ dB\end{tabular}}} & \multicolumn{2}{c|}{\textbf{Gain, dB}} & \multicolumn{2}{c|}{\textbf{Bit Pattern}} \\ \cline{3-6} 
                                                                                         &                                                                                    & \textbf{PGA}         & \textbf{ATT}        & \textbf{PGA}          & \textbf{ATT}  \\ \hline
$0$                                                                                      & $0$                                                                                & $18$                 & $-18$               & $111$                 & $000$         \\ \hline
$1$                                                                                      & $3$                                                                                & $21$                 & $-18$               & $100$                 & $000$         \\ \hline
$2$                                                                                      & $6$                                                                                & $18$                 & $-12$               & $111$                 & $001$         \\ \hline
$3$                                                                                      & $9$                                                                                & $21$                 & $-12$               & $100$                 & $001$         \\ \hline
$4$                                                                                      & $12$                                                                               & $18$                 & $-6$                & $111$                 & $011$         \\ \hline
$5$                                                                                      & $15$                                                                               & $21$                 & $-6$                & $100$                 & $011$         \\ \hline
$6$                                                                                      & $17.7$                                                                             & $26.2$               & $-8.5$              & $011$                 & $010$         \\ \hline
$7$                                                                                      & $20.5$                                                                             & $29$                 & $-8.5$              & $010$                 & $010$         \\ \hline
$8$                                                                                      & $23.5$                                                                             & $32$                 & $-8.5$              & $001$                 & $010$         \\ \hline
$9$                                                                                      & $26.5$                                                                             & $38.5$               & $-12$               & $000$                 & $001$         \\ \hline
$10$                                                                                     & $30$                                                                               & $38.5$               & $-8.5$              & $000$                 & $010$         \\ \hline
$11$                                                                                     & $32.5$                                                                             & $38.5$               & $-6$                & $000$                 & $011$         \\ \hline
$15$                                                                                     & \multicolumn{5}{c|}{Threshold crossing special code}                                                                                                                    \\ \hline
\end{tabular}
\caption{Gain settings available to AGC state machine and corresponding bit patterns for the PGA and the input attenuator. The last gain index value ($15$) is used to indicate a threshold crossing event for the corresponding channel.}
\label{tab:gain_settings}
\end{table}

% Formerly:
%\begin{table}[!ht]
%\caption{Gain values available to the AGC.}
%\label{tab:gainvalues}
%\centering
%\resizebox{0.8\textwidth}{!}{ % RESIZEBOX
%\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
%\hline
%\textbf{Gain \#} & 0 & 1 & 2 & 3 & 4  & 5  & 6    & 7    & 8    & 9    & 10 & 11   \\ \hline
%\textbf{dB}      & 0 & 3 & 6 & 9 & 12 & 15 & 17.5 & 20.5 & 23.5 & 26.5 & 30 & 32.5 \\ \hline
%\end{tabular}
%}
%\end{table}

%gain of 18 dB, 7.9, 21dB is 11.22, 12 db is 4, 6 db is 2, 8.5 db is 2.66, 26.2 db is 20.4, 29 db is 28.18, 32 db is 39.8, 38.5 db is 84,

